An Attention-based Model for Robust Forecasting with Missing Modality

Learning with missing modalities is a fundamental challenge in multimodal robot learning, as real-world robotic systems often operate in environments with incomplete sensor data. Attention-based models are appealing for processing multimodal data because they can handle multiple modalities with a single backbone network. However, most multimodal models assume that all modalities are available during both training and inference, limiting their applicability in robotic perception and decision-making. In this paper, we introduce a multimodal model designed to handle missing modalities during both training and inference. The model is formulated as a conditional variational autoencoder (CVAE) and incorporates a transformer-based architecture that leverages attention mechanisms to learn a unified, fixed-dimensional representation, even when some modalities are missing. We show that our proposed model can be trained with missing modalities while approximating a robust representation of all modalities. We evaluate our approach on five multimodal datasets across two robot learning tasks: human trajectory prediction and robot manipulation forecasting. Experimental results demonstrate that our model effectively learns from incomplete data and is superior to prior multimodal fusion approaches.

==> ICCV2025-Author-Kit-Feb/relatedwork.tex <==
\section{Related Work}

% There have been many previous works in the domain of human navigational intent inference. The majority of these studies focus on the future human motion trajectory prediction. In this section, we review previous works on human-human interaction modeling, data-driven models for trajectory prediction, and end goal-conditioned intent inference. 

\paragraph{Learning with missing modalities.}
Multimodal learning seeks to improve the performance for a task by utilizing the different available modalities, such as images, sound and natural language.  
The importance and availability of these modalities are usually not uniform. 
Therefore it is critical to have efficient multimodal fusion method for multimodal learning. Early approaches for multimodal learning are simple methods like concatenation \cite{poria2016convolutional, wang2017select}, tensor fusion \cite{zadeh2017tensor, ben2017mutan}, pooling fusions \cite{ramachandram2017deep}. 
These methods require modal-complete data, for both training and testing, which is not robust to examples with missing modalities. 
SMIL \cite{ma2021smil} proposed to reconstruct the missing modalities from a modality prior even when the training modalities are missing. \cite{ma2022multimodal} investigates the robustness of transformer model on missing-modal data and discover that the transformer model's performance drops dramatically with modal-complete data when processing all modality together using self-attention mechanism.
%\todo{we should maybe indicate the key result of the analysis}. 
However these approaches are specific to two modalities and do not extend easily to three or more modalities. 
MMF \cite{tsai2018learning} learns a joint representation of multimodal data, and perform reconstruction of missing modalities during test without significant impact on performance.
Attention mechanism has been widely studied for multimodal fusion recently \cite{nagrani2021attention, sun2019videobert}. 
Attention bottlenecks \cite{nagrani2021attention} purposed a ``fusion bottlenecks'' using cross-attention mechanism for multimodal fusion. 
Standard positional encoding is used as bottleneck tokens which only allows useful information to flow through different modalities. 
The permutation-invariant property of the transformer model has also been studied in \cite{lee2019set, tang2021sensory} and apply on set-structured data which allow the network to work with an arbitrary number of inputs. 
However, missing modality scenario was not part of their works. 
In this paper, we utilize an attention-based model to model multimodal inputs from both modal-complete and modal-incomplete data, and test it with either full or missing modality. 

% \paragraph{Human-human interaction modeling.}
% Human-human interaction is an essential feature for accurately predicting human motion behaviors in crowds. Modeling the human-human interaction has already been studied extensively in human trajectory prediction research. Early works \cite{alahi2014socially, helbing1995social, mehran2009abnormal} utilize social forces to model social interactions with attractive and repulsive forces which are based on the relative distances of agents. However,  these handcrafted features are often not robust enough for modeling complex social interactions. Therefore more recent works start using learning-based methods to model complex human behaviors. Social-LSTM \cite{alahi2016social} collects neighbouring agents’ information into a grid-based pool to capture the social interactions and Social-GAN \cite{gupta2018social} introduces a max-pooling based method to extract useful information from the surrounding neighbors. Social Ways \cite{amirian2019social} employs an attention pooling based on neighbours' pre-defined geometric features, and other attention based methods \cite{vemula2018social, sadeghian2019sophie} use learned feature vectors as the input to the attention module. Graph representations have became another popular method to model the social interaction among agents and promising results have shown especially when combing with the attention mechanism \cite{kosaraju2019social, yu2020spatio, mohamed2020social, shi2021sgcn}.


% \paragraph{Data-driven models for trajectory prediction.}
% The human trajectory prediction problem requires the data-driven models to have the ability to understand temporal data. As this is a sequence prediction task, early data-driven methods propose Recurrent Neural Networks (RNNs) such as LSTMs to encode and decode the human motion data, and these models often have deterministic outputs. More recent studies begin to develop data-driven models that produce probabilistic outputs. Multiple Generative Adversarial Network (GAN) based methods \cite{gupta2018social, sadeghian2019sophie, kosaraju2019social, amirian2019social} and Conditional Variational Autoencoder (CVAEs) models \cite{lee2017desire, mangalam2020not} have been proposed to generate multimodal future human trajectories. And to accommodate the graph representation of the social interactions, Graph Convolutional Neural Networks (GCNNs) \cite{shi2021sgcn, mohamed2020social} and Graph Attention Networks (GATs) \cite{kosaraju2019social, yu2020spatio,eiffert2020probabilistic} are implemented to learn the spatio-temporal graph representations of social agents. 

\paragraph{Multimodal human trajectory prediction.}
%Extensive research has been conducted on predicting human future trajectory, 
Early studies proposed to predict the future human trajectory based on mostly unimodal data \cite{rudenko2020human}. More recent works start to work with \textit{multimodal input} data on predicting human future trajectory. Social Ways \cite{amirian2019social} employs an attention pooling based on neighbours' pre-defined geometric features, and other attention based methods \cite{vemula2018social, sadeghian2019sophie} use learned feature vectors as the input to the attention module. 
Graph representations for multimodal input have became another popular method to model the social interaction among agents and have shown promising results.\cite{kosaraju2019social, yu2020spatio, mohamed2020social, shi2021sgcn}. Agentformer \cite{yuan2021agentformer} models the time and social information jointly with proposed agent-aware attention machanism. \cite{choi2021shared} proposes a Cross-Modal framework to learn latent space from multimodal input and test with only single input.
A majority of work \cite{yagi2018future, zhangmultimodal, rasouli2019pie, makansi2020multimodal, yao2019egocentric, yao2019unsupervised, chandra2019traphic, qiu2022egocentric} in this domain utilizes multimodal features obtained from ego-enteric view. 
%The human trajectory prediction problem requires the data-driven models to have the ability to understand temporal data. 
As human trajectory prediction is a sequential prediction task, early data-driven methods propose Recurrent Neural Networks (RNNs) such as LSTMs for predicting the trajectory, which only infer deterministic outputs. More recent studies begin to develop generative models that produce probabilistic outputs, also knowns as \textit{multimodal prediction}. Generative Adversarial Network (GAN) based methods \cite{gupta2018social, sadeghian2019sophie, kosaraju2019social, amirian2019social} and Conditional Variational Autoencoder (CVAEs) models \cite{lee2017desire, mangalam2020not} have been proposed to generate multimodal future human trajectories. However, these methods mostly work only on unimodal input, and none of existing work in human trajectory prediction domain investigates the robustness of these models against modal in-complete data.
We develop a human trajectory prediction model with transformer that can attend to every \textit{multimodal input} features, and produce \textit{multimodal prediction}.
For clarity, we use `multimodal' to only describe \textit{multimodal input} in the later of this paper. 



\begin{figure*}[t]
\begin{center}
%\fbox{\rule{0pt}{2in} \rule{.9\linewidth}{0pt}}
\includegraphics[width=0.9\textwidth]{images/figure_2.jpg}
\end{center}
\caption{Overview of our model during training (top) and inference (bottom).
The input to the multimodal encoder is a set of available modality representations obtained from the unimodal encoders (not represented in the figure). 
The multimodal encoder learns to generate a distribution over latent codes.
Then, a sampled latent code is decoded into a conditional probability distribution.
To train the model to be robust to missing modalities, the sampled latent code is decoded two times, with two sets of modalities: $\{\mathbf{x}_1,\mathbf{x}_2,\mathbf{x}_3,\mathbf{x}_5\}$ and $\{\mathbf{x}_1,\mathbf{x}_2,\mathbf{x}_5\}$.
This example shows $\mathbf{x}_3$ is removed but it can be any modalities. 
$\Sigma$ indicates the summation operator.
}
%Solid lines represent components for both training and testing. Dashed lines represent components used for training only. To generate the latent variable z during training, we use all modalities encoded by separate and independent encoders. During inference, if there are missing modalities, we use the available modalities (solid line box) to forecast the future sequence. \todo{this caption needs to be updated}}
\label{fig:overall}
\end{figure*}


\paragraph{Future goal conditioned trajectory prediction.}
Recent studies also suggest that estimating final goal before generating the entire trajectory could produce more accurate predictions \cite{zhangmultimodal}.
%While most prior works focus on predicting the entire future trajectories from beginning, some works propose to estimate the final intent or end goal of the agent first before generating or reconstructing the whole trajectories. 
\cite{rehder2018pedestrian} propose a system that first infer possible destinations of pedestrians with a mixture density function. 
%and then predict the trajectories with these destinations based on common behavior patterns. 
PRECOG \cite{rhinehart2019precog} was introduced as a multi-agent forecasting model which conditioned on one agent's goal when making predictions on other agents.
%and their experimental results show that the model's performance improve when the model is goal-conditioned. 
\cite{mangalam2020not} propose a endpoint conditioned VAE which first estimates a latent distribution based on past trajectories and future end goal.
%and then predicts a future trajectory using the plausible future goal sampled from the estimated latent distribution. 
However these methods are not able to capture the distribution of multimodal features, and produce diverse output. We show that our proposed model is able to model future goal distribution from multimodal input data, allowing our network to generate more accurate future trajectory.


% \todo{We should add the connection with our model. This section presents existing works but does not present connections with our work. Done, check?}

